Block-proximal methods with spatially adapted acceleration

We study and develop (stochastic) primal--dual block-coordinate descent methods for convex problems based on the method due to Chambolle and Pock. Our methods have known convergence rates for the iterates and the ergodic gap: $O(1/N^2)$ if each block is strongly convex, $O(1/N)$ if no convexity is present, and more generally a mixed rate $O(1/N^2)+O(1/N)$ for strongly convex blocks, if only some blocks are strongly convex. Additional novelties of our methods include blockwise-adapted step lengths and acceleration, as well as the ability to update both the primal and dual variables randomly in blocks under a very light compatibility condition. In other words, these variants of our methods are doubly-stochastic. We test the proposed methods on various image processing problems, where we employ pixelwise-adapted acceleration.

==> res/tgv2_denoising_results_lq_8000_gamma0.5_zinit_50samples.tex <==
\begin{tabular}{rr|rr|rr}
\multicolumn{6}{c}{low resolution / 0-init}\\
\hline
\multicolumn{2}{c}{gap $\le -60$dB} & \multicolumn{2}{|c}{tgt $\le -60$dB} & \multicolumn{2}{|c}{val $\le -60$dB}\\
iter & time & iter & time & iter & time\\
\hline
30 & 0.23s & 100 & 0.79s & 110 & 0.87s\\
80 & 0.46s & 200 & 1.16s & 320 & 1.87s\\
280 & 1.56s & 3380 & 18.93s & 1880 & 10.53s\\
180 & 0.81s & 340 & 1.54s & 660 & 3.00s\\
\end{tabular}


==> texbase/highlightname.tex <==
%\addbibresource{\jobname.bib}
\newcommand*{\mknamesignature}[5]{\edef#1{(#2|#3|#4|#5)}}
\mknamesignature{\highlightname}{DISABLEDValkonen}{DISABLEDTuomo}{}{}
\def\highlightfamily{Valkonen}
\def\ancientversion{2.8a}
% mbox needed to not make next character automatically  upper case
\providecommand{\shortform}{\mbox{T.\,V.}}
\makeatletter

\ifdefequal{\abx@version}{\ancientversion}{
	\DeclareNameFormat{labelname}{%
	  \begingroup
	  \mknamesignature{\currentsignature}{#1}{#3}{#5}{#7}%
	  \ifdefequal{\highlightname}{\currentsignature}%
	    {\let\mkbibnamefirst=\@gobble%
	     \def\mkbibnamelast{\shortform\@gobble}%
	     \let\mkbibnameprefix=\@gobble%
	     \let\mkbibnameaffix=\@gobble}%
	    {\let\mkbibnamefirst=\@gobble}%
	  \ifcase\value{uniquename}%
	    \usebibmacro{name:last}{#1}{#3}{#5}{#7}%
	  \or
	    \ifuseprefix
	      {\usebibmacro{name:first-last}{#1}{#4}{#5}{#8}}
	      {\usebibmacro{name:first-last}{#1}{#4}{#6}{#8}}%
	  \or
	    \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
	  \fi
	  \endgroup
	  \usebibmacro{name:andothers}%
	}
}{
	\DeclareNameFormat{labelname}{%
	  \nameparts{#1}%
	  \begingroup%
	  \mknamesignature{\currentnamex}{\namepartfamily}{\namepartgiven}{\namepartprefix}{\namepartsuffix}%
	  \ifdefstrequal{\highlightname}{\currentnamex}%
	    {%
	      \usebibmacro{name:delim}{\shortform}%
	      \shortform%
	    }{%
	      \usebibmacro{name:family}
	           {\namepartfamily}
	           {\namepartgiven}
	           {\namepartprefix}
	           {\namepartsuffix}%
	    }%
	  \endgroup%
	  \usebibmacro{name:andothers}
	}
}
\makeatother

\DeclareNameAlias{default}{labelname}


==> texbase/symbols-ip.tex <==

%\usepackage{undertilde}

\newcommand{\jprod}{\circ}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\iK}{\interior \K}
\newcommand{\E}{\mathcal{E}}
\newcommand{\Neigh}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\nullspace}[1]{\mathcal{N}(#1)}
%\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\newcommand{\Pep}{P_e^\perp}
\newcommand{\DC}{\mathrm{DC}}
\newcommand{\extsubdiff}{\widehat \subdiff}
\newcommand{\subdiffDC}{\subdiff^\DC}
\newcommand{\extsubdiffDC}{\extsubdiff^\DC}
\newcommand{\polar}[1]{{#1}^\circ}
\newcommand{\bipolar}[1]{{#1}^{\circ\circ}}
\newcommand{\regnormal}{\widehat N}
\newcommand{\regtangent}{\widehat T}
\newcommand{\HG}{{\widehat G}}
\newcommand{\HU}{{\widehat U}}
\newcommand{\IG}{\inv G}
\newcommand{\IHG}{\inv \HG}
%\newcommand{\varsym}{\bullet}
\newcommand{\wtilde}{\widetilde}
%\newcommand{\setto}{\rightrightarrows}

%\renewcommand{\norm}[1]{\|#1\|}
%\newcommand{\adjnorm}[1]{\left\|#1\right\|}

\newcommand{\eigval}{\lambda}
%\newcommand{\eigvaltwo}{\zeta}

\newcommand{\Arw}{\mathrm{Arw}}


==> texbase/symbols-mna.tex <==

\newcommand{\mna}{\phi}
\newcommand{\plusmna}{\oplus}
\newcommand{\minusmna}{\ominus}
\newcommand{\iprodmna}{\odot}
%\DeclareMathOperator{\plusmna}{\hat +}
%\DeclareMathOperator{\minusmna}{\hat{--}}
%\DeclareMathOperator{\iprodmna}{\hat \times}
\newcommand{\Rmna}{\R_\mna}
\newcommand{\maybeeq}{\stackrel{?}{=}}
\newcommand\rhodom\sqsubset
\newcommand\rhodominv\sqsupset
\newcommand\rhodomneq{\sqsubset_{!}}
\newcommand\rholub\sqcup
\newcommand\rhoglb\sqcap
\newcommand{\sumop}{\biguplus}
\newcommand{\sumz}{\biguplus}
\newcommand{\plusz}{\uplus}
\newcommand{\minusz}{\uminus}
\newcommand{\pz}{\zeta}

